Frido: Feature Pyramid Diffusion for Complex Scene Image Synthesis

Diffusion models (DMs) have shown great potential for high-quality image synthesis. However, when it comes to producing images with complex scenes, how to properly describe both image global structures and object details remains a challenging task. In this paper, we present Frido, a Feature Pyramid Diffusion model performing a multi-scale coarse-to-fine denoising process for image synthesis. Our model decomposes an input image into scale-dependent vector quantized features, followed by a coarse-to-fine gating for producing image output. During the above multi-scale representation learning stage, additional input conditions like text, scene graph, or image layout can be further exploited. Thus, Frido can be also applied for conditional or cross-modality image synthesis. We conduct extensive experiments over various unconditioned and conditional image generation tasks, ranging from text-to-image synthesis, layout-to-image, scene-graph-to-image, to label-to-image. More specifically, we achieved state-of-the-art FID scores on five benchmarks, namely layout-to-image on COCO and OpenImages, scene-graph-to-image on COCO and Visual Genome, and label-to-image on COCO. Code is available at https://github.com/davidhalladay/Frido.

==> tables/4_exp_vqgan.tex <==

\begin{table}[t]
\center
\resizebox{0.48\textwidth}{!}{
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{l|l|cc|cc}
Name & Scales & rFID & IS & PSNR & SSIM \\
\hline
VQGAN$^\dagger$ & f8 & 5.51 & 28.98 & 43.56 & 0.9554 \\
VQGAN-kl$^\dagger$ & f8 & 5.02 & \textbf{31.12} & 42.94 & 0.9548 \\
MS-VQGAN & f16f8 & \textbf{4.67} & \ul{29.31} & \textbf{44.77} & \textbf{0.9664} \\
MS-VQGAN & f32f16f8 & 6.68 & 27.67 & 44.40 & 0.9631 \\
\end{tabular}}}
\caption{Reconstruction performance comparison of quantization models. These models are trained on OpenImage 256*256 images, and evaluate on COCO-stuff valid set. $^\dagger$ denotes the model weights are loaded from the officially released codes.}
\label{exp:vqgan}
\end{table}
